Generation of Time-Varying Impedance Attacks Against Haptic Shared Control Steering Systems

The safety-critical nature of vehicle steering is one of the main motivations for exploring the space of possible cyber-physical attacks against the steering systems of modern vehicles. This paper investigates the adversarial capabilities for destabilizing the interaction dynamics between human drivers and vehicle haptic shared control (HSC) steering systems. In contrast to the conventional robotics literature, where the main objective is to render the human-automation interaction dynamics stable by ensuring passivity, this paper takes the exact opposite route. In particular, to investigate the damaging capabilities of a successful cyber-physical attack, this paper demonstrates that an attacker who targets the HSC steering system can destabilize the interaction dynamics between the human driver and the vehicle HSC steering system through synthesis of time-varying impedance profiles. Specifically, it is shown that the adversary can utilize a properly designed non-passive and time-varying adversarial impedance target dynamics, which are fed with a linear combination of the human driver and the steering column torques. Using these target dynamics, it is possible for the adversary to generate in real-time a reference angular command for the driver input device and the directional control steering assembly of the vehicle. Furthermore, it is shown that the adversary can make the steering wheel and the vehicle steering column angular positions to follow the reference command generated by the time-varying impedance target dynamics using proper adaptive control strategies. Numerical simulations demonstrate the effectiveness of such time-varying impedance attacks, which result in a non-passive and inherently unstable interaction between the driver and the HSC steering system.

==> section/AttackDesign__Alireza_Mohammadi_s_conflicted_copy_2022-11-27_.tex <==
\section{Adaptive Attack Policy}
\label{sec:attackDesign}

In this section we will design adaptive attack policies that will make the angular position of the driver's input device, i.e.,~$\theta_{\text{sw}}$, to closely follow the angular position reference $\theta_{\text{d}}$, which is generated by the target dynamical system given by~\eqref{eq:targetMain}. Our adaptive control strategy for achieving this tracking objective follows the control design proposed by Baviskar \emph{et al.}~\cite{baviskar2008adjustable}. 

We first define the driver experience error signal, i.e., the angular position tracking error between the driver input device and the target dynamics, as 
%
\begin{equation}
e_{\text{sw}} = \theta_{\text{d}} - \theta_{\text{sw}},\, 
\label{eq:errorSigsw}
\end{equation}
%
and the locked tracking error signal, i.e., the angular position tracking error between the driver input device and the steering column, as 
%
\begin{equation}
e_{\text{c}} = \theta_{\text{sw}} - \theta_{\text{c}}. 
\label{eq:errorSigc}
\end{equation}
%

Using the angular position tracking errors in~\eqref{eq:errorSigsw} and~\eqref{eq:errorSigc}, one can additionally define the filtered error signals as 
%
\begin{equation}
r_{\text{sw}} = \dot{e}_{\text{sw}} + \mu_{\text{sw}} e_{\text{sw}},\, r_{\text{c}} = \dot{e}_{\text{c}} + \mu_{\text{c}} e_{\text{c}}, 
\label{eq:filteredErr}
\end{equation}
%
where the positive gains $\mu_{\text{sw}}$ and $\mu_{\text{c}}$ are control parameters. 

To express the adaptive attack policy, in addition to the filtered error signals in~\eqref{eq:filteredErr}, we also need to define the regression matrices  
%
\begin{equation}
Y_{\text{sw}} = [Y_{N_{\text{sw}}}, -\tau_{\text{sw}}, \ddot{\theta}_{d1}  + \mu_{\text{sw}} \dot{e}_{\text{sw}}] \in \mathbb{R}^{1\times 4}, 
\label{eq:Ysw}
\end{equation}
%
and 
\begin{equation}
Y_{\text{c}} = [-Y_{N_{\text{sw}}}, \tau_{\text{sw}}, T_{\text{sw}}, Y_{N_{\text{c}}}, -\tau_{\text{c}}, \mu_{\text{c}}\dot{e}_{\text{c}}]\in \mathbb{R}^{1\times 8}, 
\label{eq:Yc}
\end{equation}
% 
where  $Y_{N_{\text{sw}}}$ and $Y_{N_{\text{c}}}$ are the regression vectors defined in~\eqref{eq:linParam}. The regression matrices $Y_{\text{sw}}$ and $Y_{\text{c}}$ consist of measurable quantities that the adversary is assumed to be able to read from the in-vehicle communication networks and/or accurately estimate. Furthermore, let us define the vectors $\phi_{\text{sw}}$, $\phi_{\text{c}}$, which stack the unknown constant parameters of the ESC steering dynamics in~\eqref{eq:dynMain} in two unknwon constant vectors, as 
%
\begin{equation}
\phi_{\text{sw}} = [\phi_{N_{\text{sw}}}, \alpha_{\text{sw}}, I_{\text{sw}}]^\top,
\label{eq:phisw}
\end{equation}
%
and
%
\begin{equation}
\phi_{\text{c}} = [\frac{I_{\text{c}}}{I_{\text{sw}}} \phi_{N_{\text{sw}}},  \frac{I_{\text{c}}}{I_{\text{sw}}} \alpha_{1}, \frac{I_{\text{c}}}{I_{\text{sw}}}, \phi_{N_{\text{c}}}, \alpha_{\text{c}}, I_{\text{c}}]^\top.  
\label{eq:phic}
\end{equation}
%
In~\eqref{eq:phisw} and~\eqref{eq:phic},  the constant unknown vectors $\phi_{N_{\text{sw}}}$ and $\phi_{N_{\text{c}}}$ are defined in~\eqref{eq:linParam}. 

Using the filtered error signals defined in~\eqref{eq:filteredErr}, the regression matrices defined in~\eqref{eq:Ysw} and~\eqref{eq:Yc}, and the constant unknown vectors defined in~\eqref{eq:phisw} and~\eqref{eq:phic}, the adversary can utilize the following control inputs 
%
\begin{equation}
T_{\text{sw}} = k_{\text{sw}} r_{\text{sw}} + Y_{\text{sw}} \hat{\phi}_{\text{sw}},\, T_{\text{c}} = k_{\text{c}} r_{\text{c}} + Y_{\text{c}} \hat{\phi}_{\text{c}}, 
\label{eq:Tattack}
\end{equation}
%
where $k_{\text{sw}}$ and $k_{\text{c}}$ are constant positive control gains, and ${\hat{\phi}}_{\text{sw}}$ and ${\hat{\phi}}_{\text{c}}$ are adaptive estimates for the unknown parameter vectors $\phi_{\text{sw}}$ and $\phi_{\text{c}}$, whose evolution are governed by the following adaptive update laws 
%
\begin{equation}
\dot{\hat{\phi}}_{\text{sw}} = \Gamma_{\text{sw}} Y_{\text{sw}}^\top r_{\text{sw}},\, \dot{\hat{\phi}}_{\text{c}} = \Gamma_{\text{c}} Y_{\text{c}}^\top r_{\text{c}},
\label{eq:adaptationLaws}
\end{equation}
%
where $\Gamma_{\text{sw}}$ and $\Gamma_{\text{c}}$ are positive constant diagonal gain matrices.


%Based on the subsequent stability analysis and the structure
% of the open-loop error system given in (9) and (10), control
% inputs $T_{\text{sw}}$ and $T_{\text{c}}$ are designed as
% and
\[
\tilde{\phi}_{\text{sw}} = \phi_{\text{sw}} - \hat\phi_{\text{sw}},\, \tilde{\phi}_{\text{c}} = \phi_{\text{c}} - \hat\phi_{\text{c}}
\]


%\[
%\dot{\hat\tau}_{\text{sw}} = -(\beta_{\text{sw}} + K_s + 1) \hat\tau_{\text{sw}} - \frac{I_{\text{sw}}}{\alpha_{\text{sw}}} \big[ (\beta_{\text{sw}}  + K_s(\beta_{\text{sw}}+1) ) \dot{e}_{\text{sw}}  + 
%K_s  \beta_{\text{sw}} e_{\text{sw}} + \rho_{\text{sw}} \text{sgn}(p_{\text{sw}})
% \big]
%\]
%
%\[
%\dot{\hat\tau}_{\text{c}} = -(\beta_{\text{sw}} + K_s + 1) \hat\tau_{\text{c}} - \frac{I_{\text{c}}}{\alpha_{\text{c}}} \big[ \rho_{\text{c}} \text{sgn}(p_{\text{c}}) 
%\big] - \frac{I_{\text{c}}}{\alpha_{\text{c}}} \big[ (\beta_{\text{sw}} + K_s(\beta_{\text{sw}}+1))\dot{e}_{\text{c}} + K_s \beta_{\text{sw}} e_{\text{c}} \big]
%\]
%
%\[
%+ \frac{I_{\text{c}}}{\alpha_{\text{c}}} \big[ \frac{\alpha_{\text{sw}}}{I_{\text{sw}}} (\dot{\hat\tau}_{\text{sw}} + (\beta_{\text{sw}}+K_s+1)\hat\tau_{\text{sw}}) \big]
%\]
%
%\[
%p_{\text{sw}} = \dot{e}_{\text{sw}} + \beta_{\text{sw}} e_{\text{sw}},\, p_{\text{c}} = \dot{e}_{\text{c}} + \beta_{\text{sw}} e_{\text{c}}
%\]
%
%
%\[
%T_{\text{sw}} = N_{\text{sw}}(\cdot) + \big(\frac{I_{\text{sw}}}{I_T}\big) (-N_T(\cdot) + \alpha_{T1} \hat\tau_{\text{sw}} + \alpha_{T2} \hat\tau_{\text{c}}) -\alpha_{\text{sw}}\hat\tau_{\text{sw}}
%\]
%
%\[
%T_{\text{c}} = N_{\text{c}}(\cdot) + \big(\frac{I_{\text{c}}}{I_{\text{sw}}}\big) (-N_{\text{sw}}(\cdot) + T_{\text{sw}} + \alpha_{1} \hat\tau_{\text{sw}}) -\alpha_{\text{c}}\hat\tau_{\text{c}}
%\]


%\section{Vehicle Traction Dynamical Model}
%\label{sec:dynmodel} 
%%
%Detailed models for the conventional and power-assisted
% steering systems exist within the literature (e.g., [5] and [22]).
% Steering models considering tire forces and vehicle dynamics have been derived in [6]. The representation of steering
% dynamics chiefly follows from the work in [5], [6], and [22].
%
%is an auxiliary nonlinear function
% that describes the dynamics on the driver side,  denotes the driver input torque, and represents a
% control input torque applied to the driver input device. denote the angular position, velocity,
% and acceleration, respectively, of the vehicle directional control
% assembly.  an auxiliary nonlinear function
% that describes the dynamics of the vehicle directional control assembly, represents the reaction torque between the
% actuator on the directional control assembly and the mechanical subsystem actuated by the directional control assembly, and . denotes the control input torque applied to the
%
%%%% driver input device; represents an auxiliary
% target dynamic function for the driver input device; and are scaling constants. The structure for (5) is
% motivated by the following philosophy: If T1(t) was exactly
%
%%%% equal to α2τ2(t) in (1), then the dynamics given by (1) offer the
% driver a realistic experience, provided that auxiliary term N1(·)
% may be designed or constructed according to some desirable
% mechanical response. Thus, the NT (·) term in (5) is designed
% to simulate the desired driving experience, and hence, this
%
%%%% dynamic equation serves as a desired trajectory generator for
% the driver input device control design.
%
%%%% 
%%%% Remark 2: The target dynamic function NT (·) must be
% selected to ensure that the desired driver input device trajectory tory and its first two derivatives remain bounded at all times.
% Suppose that NT (·) is selected as where BT and KT are some positive design constants.
% If NT (·) is designed according to (6), then standard linear
% system arguments can be used to show that θd1(t), θd1(t), and
% θd1(t) remain bounded. Furthermore, NT (·) can be constructed
% as a nonlinear damping function by utilizing Lyapunov-type
% arguments.
%%% 
%%%% INTERACTION FORCES: PART I (MEASURABLE)
% In this section, the adaptive steer-by-wire tracking controller
% is developed. The first control objective requires that both
% the target system tracking error and the locked tracking error
% signals be asymptotically regulated to zero while adapting for
% the uncertain system parameters. The control design is based
% on the assumption that the signals θ1(t), θ2(t), θ˙1(t), and θ˙2(t)
% are measurable and that driver input torque τ1(t) and the torque
% acting on the directional control system τ2(t) are measurable.
%%% 
%%%% Open-Loop Error System Development
% To quantify the mismatches between the target and primary
% systems (or driver experience tracking error), as well as the
% primary and secondary systems (or locked tracking error), the
%filtered error signals r1(t), r2(t)  are defined as
% r1 = ˙ e1 + µ1e1 r2 = ˙ e2 + µ2e2 (7)
% where µ1 and µ2 ∈ ℜ1 represent positive control gains, and
% error signals e1(t), e2(t) are
% e1 = θd1 − θ1 e2 = θ1 − θ2. (8)
% After taking the first time derivative of (7) and substituting
% the dynamics in (1) and (2), and (5) the open-loop error
% systems are
% I1r˙1 = Y1φ1 − T1 (9)
% I2r˙2 = Y2φ2 − T2 (10)
% where Y1(θ1, θ˙1, τ1, θ¨d1, θ˙d1) ∈ ℜ1×r and Y2(θ1, θ˙1, θ2, θ˙2, τ1,
% τ2, T1) ∈ ℜ1×s are regression matrices consisting of measurable quantities, and φ1  ℜr×1, φ2 are constant unknown vectors explicitly defined as follows:
%
%%%% Y1 = [YN1, −τ1, θ¨d1 + µ1e˙1] (11)
% φ1 = [φN1, α1, I1]T (12)
% Y2 = [−YN1, τ1, T1, YN2, −τ2, µ2e˙2] (13)
% φ2 = I I2 1 φN1, II21 α1, II2 1 , φN2, α2, I2T . (14)
%
%%%% 
%%%% Remark 3: Based on the definition of r1(t) and r2(t) given in
%(7), standard arguments [23] can be used to prove that 1) if r1(t)
%and r2(t) remain bounded, then e1(t), e2(t), and e˙1(t), e˙2(t)
%are also bounded, and 2) i r1(t) and r2(t) are asymptotically
% regulated, then e1(t) and e2(t) are asymptotically regulated.
%%%
%%%%In this section, we provide a brief overview of the single-wheel model of rubber-tired vehicles that are subject to  straight-ahead braking conditions. This single-wheel dynamic model can capture the steady and transient tractive performance while demonstrating how a vehicle can undergo lockup or stable braking~\cite{olson2003nonlinear,johansen2003gain,de2012torque,li2018hierarchical}. The dynamic states are often chosen to be the tire/wheel rate of  rotation and the forward vehicle speed. Hence, the quarter-car dynamics that govern the vehicle longitudinal motion during braking  are given by (see, e.g.,~\cite{johansen2003gain,de2012torque})
%%%%%
%%%%\begin{subequations}\label{eq:tractionDyn1}
%%%%	\begin{align}
%%%%	\dot{v} = -g_\alpha \mu(\lambda) - \frac{\Delta_v(t,v)}{M},\\
%%%%	\dot{\omega} = \frac{M g_\alpha r}{J} \mu(\lambda) - \frac{T_a}{J} - \frac{\Delta_w(t,\omega)}{J}, 
%%%%	\end{align}
%%%%\end{subequations}
%%%%%
%%%%\noindent where the parameters $M$, $r$, and $J$  are the quarter-car mass, wheel radius, and wheel inertia, respectively.  Additionally, during braking, the vehicle speed $v$ and the wheel rotational speed $\omega$ vary within in the set $\mathcal{D}_b:=\{ (v,\omega) | v > 0, \; 0 \leq r\omega \leq v \}$. The braking torque $T_a$ is the input to the dynamical system in~\eqref{eq:tractionDyn1}. Furthermore, the longitudinal slip $\lambda$ that determines whether the wheel is locked is given by 
%%%%%
%%%%\begin{equation}\label{eq:slipDefn}
%%%%\lambda := \frac{v- r\omega}{\max(v, r\omega)}.
%%%%\end{equation}
%%%%
%%%%%\begin{figure}
%%%%%	\centering
%%%%%	\includegraphics[scale=0.65]{./figures/gdx.png} 
%%%%%	\caption{\small Schematic of the single-wheel braking model.}
%%%%%	\label{fig:dynModel}
%%%%%\end{figure}
%%%%%%
%%%%While braking actuators are engaged, we have $\lambda = \tfrac{v- r\omega}{v}$ and $(v,\omega) \in \mathcal{D}_b$. It follows that $\lambda \in [0,1]$ during braking. We let the constant $g_\alpha$ denote $g \cos(\alpha)$ where $\alpha$ is the road slope. Finally, $\mu(\lambda)$, $\Delta_v(t,v)$, and $\Delta_w(t,\omega)$ denote the uncertain nonlinear friction coefficient, the force, and the torque disturbances resulting from unmodeled dynamics, respectively. 
%%%%
%%%%%\begin{remark}
%%%%%	\label{rem:mu}
%%%%There are a variety of ways to represent the function $\mu(\cdot)$ including the Magic Formula and Burckhardt representation (see, e.g.,~\cite{de2011optimal}). For instance, equations like Burckhardt  model (see, e.g.,~\cite{de1999model}) where 
%%%%%
%%%%\begin{equation}
%%%%\mu(\lambda) = c_1 (1-\exp(-c_2\lambda)) - c_3 \lambda,
%%%%\label{eq:burck}
%%%%\end{equation}
%%%%%
%%%%are empirical equations based on fitting coefficients that are widely utilized for modeling the interaction between the road pavement and tire tread. The longitudinal force on the tire arising from this interaction is computed by $-\mu(\lambda) g_\alpha$. 
%%%%
%%%%In this paper, we do not assume any particular closed-form representation for the nonlinear friction coefficient function $\mu(\cdot)$ and only assume that $\mu : \Lambda \to \mathbb{R}$ is a continuous function on the closed interval $\Lambda := [0,1]$. Accordingly,  $\mu(\cdot)$ attains its maximum $\mu_{\tx{max}}$ and minimum $\mu_{\tx{min}}$ on the closed interval $\Lambda$ because of the well-known properties of continuous functions on compact sets.
%%%%%\end{remark}
%%%%
%%%%It will be assumed that the disturbances $\Delta_v(t,v)$, and $\Delta_w(t,\omega)$ satisfy the following uniform bounds (see, e.g.,~\cite{de2012torque})
%%%%%
%%%%\begin{eqnarray}\label{eq:distBound}
%%%%\nonumber
%%%%|\Delta_v(t,v)| \leq \bar{\Delta}_v,\;  |\Delta_w(t,\omega)| \leq \bar{\Delta}_\omega, \\
%%%%\text{ for all } (t,v,\omega) \in [0,\infty) \times \mathcal{D}_b. 
%%%%\end{eqnarray}
%%%%
%%%%It is possible to transform the longitudinal dynamics by a change of coordinates from $(v,\omega)$ to $(v, \lambda)$. Under this change of coordinates, the longitudinal dynamics become (see, e.g.,~\cite{de2012torque,olson2003nonlinear} for the details of derivation) 
%%%%\begin{subequations}\label{eq:tractionDyn2}
%%%%	\begin{align}
%%%%	\dot{v} &= -g_\alpha \mu(\lambda) - \frac{\Delta_v(t,v)}{M},\\
%%%%	\dot{\lambda} &= \frac{g_\alpha}{v}\big\{ (\lambda - 1 - \nu) \mu(\lambda) + \Upsilon_a + \Upsilon_{\Delta, w} + (\lambda -1)\Upsilon_{\Delta, v} \big\}, 
%%%%	\end{align}
%%%%\end{subequations}
%%%%\noindent where $\nu:=\tfrac{M R^2}{J}$ is the dimensionless ratio of vehicle to wheel inertia, $\Upsilon_a := \frac{r}{J g_\alpha} T_a$ is the dimensionless brake torque, and $\Upsilon_{\Delta, w} := \frac{r}{J g_\alpha} \Delta_w(t, \omega)$, $\Upsilon_{\Delta, v} := \frac{\Delta_v(t,v)}{M g_\alpha}$ are the dimensionless force and torque disturbances acting on speed and slip dynamics, respectively. 
%%%%
%%%%The dynamical equations in~\eqref{eq:tractionDyn1} and~\eqref{eq:tractionDyn2} capture the coupling in-between the wheel slip $\lambda$ dynamics with that of the vehicle speed $v$ in case of~\eqref{eq:tractionDyn2}, or the tire/wheel angular speed $\omega$ dynamics with that of the vehicle speed $v$ in case of~\eqref{eq:tractionDyn1}. In $(v, \lambda)$ coordinates, the set  $\mathcal{D}_b$ reads as 
%%%%%
%%%%\begin{equation}
%%%%\mathcal{D}_b=\big\{ (v,\lambda) | v > 0, \; \lambda \in \Lambda := [0,1] \big\}.
%%%%\label{eq:Db}
%%%%\end{equation}
%%%%%
%%%% 
%%%% Using the brake input $\Upsilon_a$, the adversary would like to induce unstable braking conditions corresponding to lockup. The most severe case of lockup happens when $\lambda=1$. Therefore, following Olson \emph{et al.}~\cite{olson2003nonlinear}, we define \textbf{the lockup manifold} in the following way
%%%%%
%%%%\begin{equation}
%%%%\mathcal{W}_b^L := \big\{ (v,\lambda) \big| v>0,\, \lambda = 1 \big\}.
%%%%\label{eq:lockupManifold}
%%%%\end{equation}
%%%%%
%%%%\begin{remark}
%%%%	It is remarked that the adversary can choose the slip reference value $\lambda^{\text{r}}$ in advance, which can belong to the interval $[0,1]$.  The closer $\lambda^{\text{r}}$ to one, the closer the wheel to the condition of lockup. Without loss of generality, we assume that $\lambda^{\text{r}}$ has been chosen to be equal to one. 
%%%%\end{remark}
%%%%
%%%%To model the adversarial disruption resources, we assume that the reference malicious command generated by the attack policy $\hat{\Upsilon}_a$ passes through the following first-order delay system (see, e.g.,~\cite{de2012torque,li2018hierarchical})  
%%%%%
%%%%\begin{equation}
%%%%\tau_f \dot{\Upsilon}_a  = - \Upsilon_a + \hat{\Upsilon}_a(t- \delta_f), 
%%%%\label{eq:torqueResp}
%%%%\end{equation}
%%%%% 
%%%%to generate the frictional braking torque response $\Upsilon_a$, which then gets applied to the traction dynamics in~\eqref{eq:tractionDyn2}.  It is remarked that the attacker does not have any knowledge of either the friction brake time constant $\tau_f$ or the friction brake deadtime $\delta_f$. In designing our attack policies in the next section, we assume that $\tau_f \approx 0$ and $\delta_f \approx 0$. However, the simulation results in Section~\ref{sec:sims} demonstrate the effectiveness of the attack policies when these assumptions do not hold.

%In this section, we present an attack policy that can achieve the wheel lockup attack policy objective in the previous section. The proof of the stated propositions are removed for the sake of brevity. The  attack policy relies on a feedback and a feedforward control action. The feedback control input is generated through a predefined-time controller~\cite{sanchez2015predefined} that can cause wheel lockups if the tire-road interaction characteristics and other relevant parameters in the vehicle traction dynamics are completely known. Against the lack of such information,  it is shown that the  adversary can employ an additional feedforward control input that is generated by a nonlinear disturbance observer. %The NDOB will compensate for the adversarial limited knowledge of the vehicle traction dynamics. 
%%We start with a simple attack policy based on the concept of predefined-time controllers proposed in~\cite{sanchez2015predefined} and assume that %the adversary has an almost perfect knowledge of the vehicle dynamics. 
%%The sophistication level of the attack policy analysis and design by assuming less knowledge of the dynamical model. 
%
%\noindent\textbf{Predefined-time controller design.} Following the notation in~\cite{sanchez2015predefined}, we let 
%%
%\begin{equation}
%\Phi_p(x):=\frac{\exp(|x|^p)}{p} |x|^{1-p} \tx{sign}(x),  
%\label{eq:phip}
%\end{equation}
%%
%for any $x\in \mathbb{R}$ and some real constant $0 < p < 1$, and   
%\begin{equation}
%\Phi_1(x):=\exp(|x|) \tx{sign}(x),
%\label{eq:phi1}
%\end{equation}
%%
%for any $x\in \mathbb{R}$. Furthermore, we define the lockup error as
%%
%\begin{equation}
%\label{eq:eL}
%e_L := \lambda - 1. 
%\end{equation}
%%
%\noindent Hence, if $e_L=0$ and $v>0$, the wheel is in a locked stated. As it will be demonstrated in this section, if the attack objective is met, the wheel will be locked in finite time. Hence, the vehicle speed will satisfy  
%%
%\begin{equation}
%\label{eq:speedBound}
%v \in [v_\tx{min}, v_\tx{max}], 
%\end{equation}
%%  
%during a successful attack, for some positive $v_\tx{min}$ and $v_\tx{max}$. 
%%Using the functions defined in~\eqref{eq:phip} and~\eqref{eq:phi1}, we define the following 
%%feedback control laws 
%%%
%%\begin{eqnarray}
%%u_{np}^a(e_\tx{L}) &:=& -k_a \tx{sign}(e_L) -\frac{1}{T_c} \Phi_p(e_L), 
%%\label{eq:unp}
%%\\
%%u_{n1}^a(e_\tx{L}) &:=& -\big(\frac{1}{T_c} + k_a \big) \Phi_1(e_L),
%%\label{eq:un1}
%%\end{eqnarray}
%%%
%%\noindent where $k_a$, $T_c$, and $0<p<1$  are some positive real constants. 
%%
%\begin{proposition}
%	\label{prop:prop1}
%	Consider the vehicle longitudinal dynamics $\mathcal{P}$ in~\eqref{eq:tractionDyn2} with the attacker's \emph{a priori} knowledge $\hat{\mathcal{P}}$ in~\eqref{eq:tractionDyn2approx} and the frictional braking response given by~\eqref{eq:torqueResp} with $\tau_f \approx 0$ and $\delta_f \approx 0$.  Suppose $\Upsilon_{\Delta, w}=0$, $\hat{\nu}=\nu$, and $\hat{\mu}(\cdot)=\mu(\cdot)$. Additionally, assume that the uniform bound on $\Delta_v(t,v)$ given by~\eqref{eq:distBound} holds. Given any positive constant $T_c$, the attack policy
%	\begin{equation}
%	\label{eq:attPolicyNoDob}
%	\hat{\Upsilon}_a = \frac{v}{g_\alpha} u_{np}^a(e_\tx{L}) + \hat{\nu} \hat{\mu}(\lambda),  
%	\end{equation}
%	with $u_{np}^a(e_\tx{L})=  -(\tfrac{1}{T_c} + k p ) \Phi_p(e_L)$, where $0 < p < 1$, $k \geq k^{\ast\prime}:=\tfrac{M g_\alpha \mu_{\max} + \bar{\Delta}_v}{M v_{\tx{min}}}$, and $\Phi_p(\cdot)$ given by~\eqref{eq:phip}, makes the lockup manifold $\mathcal{W}_b^L$  globally finite-time stable with settling-time $T_c$. 
%\end{proposition}
%
%%\noindent\textbf{Proof.} The closed-loop dynamics of $e_L$ under the stated assumptions become  
%%\begin{equation}\label{eq:errorDyn0}
%%\dot{e}_L  =   u_{np}^a(e_\tx{L})  + \Delta_e(t,e_L),  
%%\end{equation}
%%%
%%\noindent where $\Delta_e(t,e_L) = \tfrac{g_\alpha}{v} e_L \{\mu(\lambda) + \Upsilon_{\Delta, v} \}$ is a vanishing 
%%perturbation satisfying $|\Delta_e(t,e_L)| \leq \tfrac{M g_\alpha \mu_{\max} + \bar{\Delta}_v}{M v_{\tx{min}}} |e_L|$. Therefore, 
%%by Lemma~4.1 in~\cite{sanchez2015predefined}, the proposition is proved.\hfill$\blacksquare$
%
%\begin{remark}
%Proposition~\ref{prop:prop1} assumes an almost perfect knowledge of the vehicle's model, where the only unknown is the 
%disturbance force $\Delta_v(t,v)$ acting on the vehicle speed dynamics in~\eqref{eq:tractionDyn2}. The next proposition 
%removes these restrictions further.  
%\end{remark} 
%
%\begin{proposition}
%	\label{prop:prop2}
%	Consider the stated assumptions in Proposition~\ref{prop:prop1} with $\hat{\nu}$ arbitrary, and     $\Delta_w(t,\omega)$, $\Delta_v(t,v)$ satisfying~\eqref{eq:distBound}. Furthermore, assume  that $\hat{\mu}: \Lambda \to \mathbb{R}$ is a continuous function. Then, given $0 < T_c < 1$, the attack policy~\eqref{eq:attPolicyNoDob} with $u_{np}^a(e_\tx{L})=  -k_a \tx{sign}(e_L) -\tfrac{1}{T_c} \Phi_p(e_L)$, $0 < p < 1$, $\Phi_p(\cdot)$ given by~\eqref{eq:phip}, and $k_a \geq k^\ast$ in which  
%	\begin{equation}
%	\label{eq:kBound}
%		k^\ast := \frac{M g_\alpha \mu_{\max} + \bar{\Delta}_v}{M v_{\tx{min}}} + \frac{g_\alpha}{v_{\tx{min}}}\big( \hat\nu \hat\mu_{\text{max}} + \nu \mu_{\text{max}} + \frac{r \bar{\Delta}_w}{J g_\alpha} \big), 
%	\end{equation}
%	makes the lockup manifold $\mathcal{W}_b^L$ globally finite-time stable with settling-time $T_c$. 
%\end{proposition}
%
%
%%\noindent\textbf{Proof.} The closed-loop dynamics of $e_L$ under the stated assumptions read as 
%%	\begin{equation}\label{eq:errorDyn2}
%%	\dot{e}_L  =   u_{np}^a(e_\tx{L})   + \Delta_e^{\prime}(t,e_L),   
%%	\end{equation}
%%	% 
%%	\noindent where 
%%	\begin{eqnarray}
%%	\nonumber
%%	\Delta_e^{\prime}(t,e_L) & = & \frac{g_\alpha}{v} e_L \big\{\mu(\lambda) +  \Upsilon_{\Delta, v}  \big\} + \cdots \\
%%    &  & \frac{g_\alpha}{v} \big\{\hat{\nu}\hat{\mu}(\lambda) - \nu\mu(\lambda)\big\} + \frac{g_\alpha}{v} \Upsilon_{\Delta, w},
%%	\label{eq:kbound2}
%%	\end{eqnarray}
%%	%  
%%	is a non-vanishing perturbation. Due to the definition of wheel slip, we have $|e_L| \leq 1$ for all values of $\lambda \in \Lambda$. Therefore, it follows that $|\Delta_e^{\prime}(t,e_L)| \leq k^\ast$, where $k^\ast$ is given by~\eqref{eq:errorDyn2}. Consequently, 
%%	by Lemma~4.3 in~\cite{sanchez2015predefined}, the proposition is proved.\hfill$\blacksquare$
%
%The following proposition, whose proof is omitted for the sake of brevity, removes the restrictions on the settling-time in Proposition~\ref{prop:prop2}. 
%
%\begin{proposition}
%Consider the stated assumptions in Proposition~\ref{prop:prop2}. Given any positive constant $T_c$, the attack policy 
%\begin{equation}
%\label{eq:attPolicyNoDob3}
%\hat{\Upsilon}_a = \frac{v}{g_\alpha} u_{n1}^a(e_\tx{L}) + \hat{\nu} \hat{\mu}(\lambda),  
%\end{equation}
%with $u_{n1}^a(e_\tx{L})=  -(\tfrac{1}{T_c} + k_a) \Phi_1(e_L)$, where $k_a \geq k^\ast$, $k^\ast$ given by~\eqref{eq:kBound}, and $\Phi_1(\cdot)$ given by~\eqref{eq:phi1}, makes the lockup manifold $\mathcal{W}_b^L$ globally finite-time stable with  settling-time $T_c > 0$.  
%\label{prop:prop3}	
%\end{proposition}
%%
%%
%%\begin{eqnarray}\label{eq:errorDyn}
%%\nonumber
%%\dot{e}_L & =   \frac{g_\alpha}{\hat{g}_\alpha} u_n^a(e_\tx{L}) - \frac{g_\alpha}{v} \hat{d}_a  + \frac{g_\alpha}{v} e_L \big\{\mu(\lambda) + \Upsilon_{\Delta, v}  \big\} + \\
%%& \frac{g_\alpha}{v} \big\{\hat{\nu}\hat{\mu}(\lambda) - \nu\mu(\lambda)\big\} + \frac{g_\alpha}{v} \Upsilon_{\Delta, w} 
%%\end{eqnarray}
%%locally finite-time convergent to a compact set $\Omega_b^L$ containing $\mathcal{W}_b^L$ such that $|e_L| \leq f(| d |_\infty)$. 
%%
%\noindent\textbf{Nonlinear disturbance observer design.} Thus far, the presented family of attack policies in Propositions~\ref{prop:prop1}--\ref{prop:prop3} depend on some \emph{a priori} knowledge of the vehicle  longitudinal dynamics $\mathcal{P}$ in~\eqref{eq:tractionDyn2}. Against the lack of such information in realistic scenarios, we add a feedforward compensation term to the proposed attack policies. In particular, we extend the brake attack policies in~\eqref{eq:attPolicyNoDob} and~\eqref{eq:attPolicyNoDob3} according to 
%%
%\begin{equation}
%\label{eq:attPolicyDob}
%\hat{\Upsilon}_a = \frac{v}{g_\alpha} u_{ni}^a(e_\tx{L}) + \hat{\nu} \hat{\mu}(\lambda) - \hat{d}_a, \; i=1,\, p, 
%\end{equation}
%%
%where $\hat{d}_a \in \mathbb{R}$ is the output of the following NDOB (see, e.g.,~\cite{chen2004disturbance,mohammadi2017nonlinear} for details of derivation)
%%
%\begin{subequations}\label{eq:dobDyn}
%	\begin{align}
%	\dot{z}_a &= -L_d z_a - L_d \big\{ u_{ni}^a + \frac{g_\alpha}{v} (-\hat{d}_a + 
%	\hat{\nu}\hat{\mu}(\lambda)  + p_a) \big\},\\
%	\hat{d}_a &= z_a + p_a, 
%	\end{align}
%\end{subequations}
%%
%\noindent where $z_a \in \mathbb{R}$ is the state of the NDOB, and the relationship $p_a = L_d e_L$ between $L_d$, namely, the 
%NDOB gain, and $p_a$, namely, the NDOB auxiliary variable, holds. 
%%
%%\begin{equation}
%%\label{eq:pLrel}
%%p_a = L_d e_L,   
%%\end{equation}
%%
%\noindent Therefore, it follows that $L_d = \tfrac{\partial p_a}{\partial e_L}$. 
%
%%The NDOB in~\eqref{eq:dobDyn}  has been designed based on considering the wheel slip error dynamics 
%%%
%%\begin{equation}\label{eq:errorDyn3}
%%\dot{e}_L  =   u_{ni}^a(e_\tx{L})   + \Delta_e^{\prime}(t,e_L) - \hat{d}_a, \, i=1,\, p,   
%%\end{equation} 
%%% 
%%where $\Delta_e^{\prime}(t,e_L)$ denotes the lumped disturbance. The NDOB output $\hat{d}_a$, which is being calculated by~\eqref{eq:dobDyn}, tries to cancel the lumped disturbance $\Delta_e^{\prime}(t,e_L)$. In the ideal case, when $\hat{d}_a \approx \Delta_e^{\prime}(t,e_L)$, complete disturbance cancellation is achieved and it appears to the predefined-time controller, which was designed in Step~1, that it is controlling a system with no disturbances. The block diagram of the proposed attack policy is depicted in Figure~\ref{fig:blockDiag1}. 
%
%\begin{figure}
%	\centering
%	\includegraphics[scale=0.40]{./figures/gdx1.png} 
%	\caption{The proposed attack policy block diagram.}
%	\label{fig:blockDiag1}
%\end{figure}
%
%The convergence properties of the disturbance tracking error are well-studied in the literature (see, e.g.,~\cite{li2014disturbance,chen2004disturbance,mohammadi2017nonlinear}) and for the sake of brevity we refer the readers to the aforementioned references. 
%
%\begin{remark}\label{rem:choice}
%	The NDOB in~\eqref{eq:dobDyn} has only one dynamic state and it does not rely on having a particular representation such as the Burckhardt closed-form for the nonlinear friction coefficient function $\mu(\cdot)$. Indeed, whenever no knowledge of $\mu(\cdot)$ is available, the adversary can set $\hat{\mu}(\lambda)$ to be equal to zero in~\eqref{eq:dobDyn}.   This NDOB-based disturbance compensation technique is unlike the adaptive algorithms in~\cite{de2012torque,li2018hierarchical} where a particular representation of the friction coefficient function is needed and several parameters need to get updated simultaneously. As it will be seen in the simulations, even when $\hat{\mu}(\lambda)$ is set to zero, corresponding to a complete lack of knowledge by the adversary, the attack policy using the NDOB will meet its objectives. 
%\end{remark}



==> section/AttackPolicy.tex <==
\section{Attack Policy Objectives}
\label{sec:AttackPolicy}
%
In this section we formulate the attack policy objectives and state our assumptions about the adversarial knowledge of 
the vehicle dynamical model. 

Following  the notation by Teixeira \emph{et al.}~\cite{teixeira2015secure}, we denote the vehicle traction dynamics in~\eqref{eq:tractionDyn2} by $\mathcal{P}$. Moreover, we let the attacker's \emph{a priori}  knowledge model $\hat{\mathcal{P}}$ be given by 
%
\begin{subequations}\label{eq:tractionDyn2approx}
	\begin{align}
	\dot{v} = -{g}_{\alpha} \hat{\mu}(\lambda),\\
	\dot{\lambda} = \frac{{g}_\alpha}{v}\big\{ (\lambda - 1 - \hat{\nu}) \hat{\mu}(\lambda) + \hat{\Upsilon}_a \big\}, 
	\end{align}
\end{subequations}
%
\noindent where the adversary has no \emph{a priori knowledge} of the dimensionless torque and force disturbances $\Upsilon_{\Delta, w}$, $\Upsilon_{\Delta, v}$. Furthermore, the adversary has only an approximate knowledge of the tire-road interaction characteristics given by $\hat{\mu}(\lambda)$. When the adversary does not have any knowledge of $\mu(\lambda)$, the friction coefficient $\hat{\mu}(\lambda)$ is set equal to $0$ in $\hat{\mathcal{P}}$.  We assume that the adversary knows and/or can compute the vehicle velocity as well as the wheel slip. This scenario corresponds to having complete access to disclosure resources in the cyber-attack space~\cite{teixeira2015secure}. 
%Indeed, as demonstrated in an experimental wireless attack against Tesla vehicles~\cite{nie2017free}, an adversary who has the capability of %reprogramming the firmware of ECUs through the Unified Diagnostic Services (UDS) codified in ISO-14229~\cite{iso14229} can also read live data from %the IVN (such as vehicle speed or engine speed). 

\noindent\textbf{Wheel Lockup Attack Policy Objective.} Given the vehicle longitudinal dynamics $\mathcal{P}$ in~\eqref{eq:tractionDyn2}, the attacker's \emph{a priori} knowledge $\hat{\mathcal{P}}$ in~\eqref{eq:tractionDyn2approx}, and the  braking response in~\eqref{eq:torqueResp}, design an attack policy $\hat{\Upsilon}_a$ such that the trajectories of the vehicle longitudinal dynamics during braking converge to any sufficiently close neighborhood of the lockup manifold  $\mathcal{W}_b^L$ within a finite time interval. 

==> section/CLFQP.tex <==
\section{CLF-based Quadratic Program Solution}

\begin{itemize}
	\item This is the trivial solution after the zero dynamics analysis 
	is done. However, it lacks a proper geometric insight. Indeed, this control 
	strategy makes the robot to converge to the zero dynamics manifold in a direction perpendicular 
	to the manifold.  
\end{itemize}

==> section/ContProbFormulation.tex <==
\section{Adversary Model and Attack Policy Objectives}
\label{sec:AttackPolicy}







==> section/ODSQP.tex <==
\section{Attack Policy Design}
\label{sec:attackDesign}


\[
\Upsilon_a = \frac{v}{g_\alpha} u_n^a(e_\tx{L}) + \hat{\nu} \hat{\mu}(\lambda) - \hat{d}^a
\]

\[
e_L = \lambda - 1 
\]

\begin{eqnarray}\label{eq:errorDyn}
\nonumber
\dot{e}_L & =  u_n^a(e_\tx{L}) - \frac{g_\alpha}{v} \hat{d}_a  + \frac{g_\alpha}{v} e_L \big\{\mu(\lambda) + \Upsilon_{\Delta, v}  \big\} + \\
& \frac{g_\alpha}{v} \big\{\hat{\nu}\hat{\mu}(\lambda) - \nu\mu(\lambda)\big\} + \frac{g_\alpha}{v} \Upsilon_{\Delta, w} 
\end{eqnarray}

\[
u_n^a(e_\tx{L}) = -\big(\frac{1}{T_c} + k_a \big) \Phi_1(e_L)
\]

\[
u_n^a(e_\tx{L}) = -k_a \frac{e_L}{| e_L |} -\frac{1}{T_c} \Phi_p(e_L)
\]

\[
\tau_f \dot{T}_a^{\ast}  = - T_a^{\ast} + T_a(t- \delta_f)
\]


\begin{subequations}\label{eq:dobDyn}
	\begin{align}
	\dot{z}_a &= -L_d(t)z_a - L_d(t) \big\{ u_n^a + \frac{g_\alpha}{v} (-\hat{d}_a + 
	\hat{\nu}\hat{\mu}(\lambda)  + p) \big\},\\
	\hat{d}_a &= z_a + p
	\end{align}
\end{subequations}

\[
p(t) = L_d(t) e_L 
\]



==> section/header2.tex <==
% Header.tex

\usepackage{array,pdfsync,enumerate,tikz,enumerate}
\usepackage[dvips]{epsfig}
\usepackage{amssymb,amsmath}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{multirow}
%
\usepackage{color}
\definecolor{linkcol}{rgb}{0,0.0,1.0}
\definecolor{citecol}{rgb}{0.0,0.6,0.0}


\IEEEoverridecommandlockouts
% The preceding line is only needed to identify funding in the first footnote. If that is unneeded, please comment it out.
\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
%\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
%		T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

%\overrideIEEEmargins
%\IEEEoverridecommandlockouts                              % This command is only
%\usepackage{macros,macros2}


\usepackage{hyperref}
\hypersetup{colorlinks,breaklinks,
	linkcolor=linkcol,urlcolor=citecol,
	anchorcolor=linkcol,citecolor=citecol,bookmarks=true}
%----------------------------------
\newcounter{MYtempeqncnt}
\usepackage{caption}
\usepackage{subcaption}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\thbf}{\boldsymbol\theta}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\rank}{rank}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% %----------------------------
%% % THEOREMS
%% % ---------------------------------------------------------------
%% %%%%%%%%%%%%%%%%%%%%%%%
%\theoremstyle{definition}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{defi}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
%%\newtheorem{assumption}[theorem]{Assumption}
%\newtheorem{exmple}[theorem]{Example}
%\newcommand{\tx}[1]{\text{#1}}
%%\newtheorem{procedure}[theorem]{Procedure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newenvironment{example}{
%	\begin{exmple}\rm}{\hfill $\bigtriangleup$%
%	\end{exmple}
%}
%
%\newenvironment{remark}{
%	\begin{rmrk}\rm}{ \hfill{ }$\bigtriangleup$%
%	\end{rmrk}
%}
%
%
%\newenvironment{definition}{
%	\begin{defi}\rm}{\hfill $\bigtriangleup$%
%	\end{defi}
%}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\renewcommand\thetheorem{\arabic{section}.\arabic{theorem}}
%
%\title{\Large \bf }
%==============================================
\newcommand{\rpos}{\mathbb{R}_{\geq 0}}
\newcommand{\ex}{\hat{e}_x}
\newcommand{\ez}{\hat{e}_z}
\newcommand{\ethr}{\hat{e}_{\theta_r}}
\newcommand{\ethrp}{\hat{e}^{\perp}_{\theta_r}}
\newcommand{\tx}[1]{\text{#1}}

\usepackage{graphicx}      % include this line if your document contains figures
\usepackage{cite}
%\usepackage{natbib}        % required for bibliography
%===============================================================================
\renewcommand\floatpagefraction{.9}
\renewcommand\dblfloatpagefraction{.9} % for two column documents
\renewcommand\topfraction{.9}
\renewcommand\dbltopfraction{.9} % for two column documents
\renewcommand\bottomfraction{.9}
\renewcommand\textfraction{.1}   
\setcounter{totalnumber}{50}
\setcounter{topnumber}{50}
\setcounter{bottomnumber}{50}
%================================================================================
\begin{document}
	
	\title{Investigation of Wheel Lockup Attacks on Nonlinear Dynamics of Vehicle Traction Using
		Frictional Brakes}
	
	\author{Alireza Mohammadi and Hafiz Malik\\% <-this % stops a space
		Emails: {\tt \{amohmmad,hmalik\}@umich.edu}
		%\thanks{This work was not supported by any organization}% <-this % stops a space
		%\thanks{%This work is supported by NSF Award 2035770. A. Mohammadi and H. Malik are with the
			%Department of Electrical and Computer Engineering, University of Michigan-Dearborn, MI 48127 USA. M. Abbaszadeh is with 
			%GE Global Research, NY 12309 USA.  
		%	Emails: {\tt\small \{amohmmad,hmalik\}@umich.edu}.}%
	}
	

\maketitle		
		
%		\begin{abstract}                % Abstract of not more than 250 words.
%			 There is ample evidence in the automotive cybersecurity literature that the car brake ECUs can be maliciously reprogrammed. 
%			 Motivated by such threat, this paper investigates the capabilities of an adversary who can directly control the frictional brake actuators and would like to induce wheel lockup conditions leading to catastrophic road injuries.  Simulations under various road conditions demonstrate the effectiveness of the proposed attack policy.          
%		\end{abstract}
		
	%	\begin{keyword}
	%	quadratic programming, autonomous robots, nonlinear control systems, saturation, guidance systems.
	%	\end{keyword}
		
		
		
%	\end{frontmatter}

%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%\include{PhDBiblio}	
%===============================================================================

==> section/miscSteering.tex <==
My note: reducing the driving load; transition from autonomy to manual; increasing the joyful experience of driving

@incollection{abbink2010neuromuscular,
	title={Neuromuscular Analysis as a Guideline in designing Shared Control},
	author={Abbink, DA and Mulder, M},
	booktitle={Advances in Haptics},
	pages={499--516},
	year={2010},
	publisher={Intech}
}


@article{nekouei2021randomized,
	title={A randomized filtering strategy against inference attacks on active steering control systems},
	author={Nekouei, Ehsan and Pirani, Mohammad and Sandberg, Henrik and Johansson, Karl H},
	journal={IEEE Transactions on Information Forensics and Security},
	volume={17},
	pages={16--27},
	year={2021},
	publisher={IEEE}
}


% Dawson papers: 
@inproceedings{mandhata2012evaluation,
	title={Evaluation of a customizable haptic feedback system for ground vehicle steer-by-wire interfaces},
	author={Mandhata, Uday B and Jensen, Matthew J and Wagner, John R and Switzer, Fred S and Dawson, Darren M and Summers, Joshua D},
	booktitle={2012 American Control Conference (ACC)},
	pages={2781--2787},
	year={2012},
	organization={IEEE}
}


@article{baviskar2008adjustable,
	title={An adjustable steer-by-wire haptic-interface tracking controller for ground vehicles},
	author={Baviskar, Abhijit and Wagner, John R and Dawson, Darren M and Braganza, David and Setlur, Pradeep},
	journal={IEEE Transactions on Vehicular Technology},
	volume={58},
	number={2},
	pages={546--554},
	year={2008},
	publisher={IEEE}
}


% The raw material for paper writing: 
@inproceedings{ferraguti2013tank,
	title={A tank-based approach to impedance control with variable stiffness},
	author={Ferraguti, Federica and Secchi, Cristian and Fantuzzi, Cesare},
	booktitle={2013 IEEE international conference on robotics and automation},
	pages={4948--4953},
	year={2013},
	organization={IEEE}
}

Humans interact with the surrounding environment constantly, e.g. moving an utensil, catching a ball, opening a door. The growing interest in reproducing human-like behavior in many robotic tasks brought the control of the interaction between a manipulator and the environment to be a key component for the success of many manipulation tasks. These interactions may often be unstable, especially when the task involves a tool.

The concept of active control of a manipulator’s interactive behavior is formally treated as an aspect of impedance control [2]. The impedance control provides a compliant behavior during the interaction and regulates the dynamic response of the robot end-effector to interaction forces by establishing a suitable virtual mass-spring-damper system on the end-effector.

Excessive contact force between the manipulator and the environment should be prevented. Since humans control the force exerted on an object by adapting their arm stiffness, in a similar way the robot should be able to change the stiffness of its arm while performing an interaction task. In this paper we presented a passivity-based impedance control algorithm with variable stiffness. The passification strategy involves the exploitation of an energy tank that store back the energy dissipated by the system.

~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

@article{kronander2016stability,
	title={Stability considerations for variable impedance control},
	author={Kronander, Klas and Billard, Aude},
	journal={IEEE Transactions on Robotics},
	volume={32},
	number={5},
	pages={1298--1305},
	year={2016},
	publisher={IEEE}
}

Variable impedance control allows not only controlling the dynamic relationship between external forces and robot movements, but in addition gives the flexibility to change these dynamics in a continuous manner during the task.

There is hence a need for analysis or control methods that can guarantee stable execution of variable impedance tasks. This
issue has been recently addressed in [8], wherein a tank-based approach to passive varying stiffness was proposed. Their system uses the total energy of the manipulator (kinetic plus virtual potential energy coming from stiffness term), but does not constrain this function to strictly decrease. Instead, any dissipated energy is added to a virtual energy tank, from which energy can be extracted in order to implement stiffness variations. The tank is given an initial level of energy and a maximum allowed level of energy. These levels determine to what extent the system will accept stiffness variations. 

It has two important shortcomings, which are as follows. 1) It depends on the state of the robot, with the consequence that
one cannot guarantee beforehand the execution of a desired
impedance profile. 2) The performance depends strongly on the intial and threshold
levels of energy in the tank. 

Our aim with this work is to provide a stability condition for varying stiffness and damping that is state independent. The
most important practical advantage of such a constraint is that it can be verified offline, before execution of the task. Any standard impedance control architecture can subsequently be used for task execution, with a reassuring guarantee that the system cannot go unstable.

We focus on variable stiffness and damping, which are the impedance parameters that are most commonly varied for im-
proving task performance. We then propose a stability condition that relates the stiffness, damping, and their rates of change. The constraint arises from the choice of a Lyapunov candidate function in which mixed position and velocity terms appear in the time derivative. Our main contribution in this paper is using this function to derive stability constraints for stiffness and damping profiles, and evaluating how these constraints can be used in practice.

~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

@article{lazcano2021mpc,
	title={MPC-based haptic shared steering system: a driver modeling approach for symbiotic driving},
	author={Lazcano, Andrea Michelle Rios and Niu, Tenghao and Akutain, Xabier Carrera and Cole, David and Shyrokau, Barys},
	journal={IEEE/ASME Transactions on Mechatronics},
	volume={26},
	number={3},
	pages={1201--1211},
	year={2021},
	publisher={IEEE}
}

The exponential growth of advanced driver assistance systems  the years has a direct impact on increased safety and reduction of mental workload while driving [1]. However, automation can also lead to unsatisfactory user acceptance when the driver's intention or expectation does not match the behavior of the driving assist system [2]. Moreover, the different projections toward the d ems (ADAS) over the years. 

The shared control approach is particularly suitable for the steering task as forces can be exchanged at the steering wheel to accomplish a common objective. Through haptic shared control (HSC), the authority of the driving task is balanced between the driving assist system and the driver. However, although HSC can lead to less steering control activity and increased safety [4], drivers sometimes resist the assist system’s guidance [5]. This can be due to, for example, a mismatch between the driver's cognitive intentions and the controller's objective, or, from a neuromuscular level, the reflex action of the muscle spindles [6].

The introduction of the steering system dynamics is key to investigate the interaction between driver and driving assist system. The steering dynamics are rigidly coupled to the arms dynamics at the steering wheel, where torques are exchanged.

Thereby resulting in a lumped inertia that is the sum of the inertia of the arms Iarms and the inertia of the steering wheel Isw. The neuromuscular dynamics of the arms are described in detail in Section III-B. The proposed control strategy tackles the need to blend driver and assist system through driver modeling in an HSC strategy. 

~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

@article{lv2021human,
	title={Human--Machine Collaboration for Automated Driving Using an Intelligent Two-Phase Haptic Interface},
	author={Lv, Chen and Li, Yutong and Xing, Yang and Huang, Chao and Cao, Dongpu and Zhao, Yifan and Liu, Yahui},
	journal={Advanced Intelligent Systems},
	volume={3},
	number={4},
	pages={2000229},
	year={2021},
	publisher={Wiley Online Library}
}

~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

@article{mars2014analysis,
	title={Analysis of human-machine cooperation when driving with different degrees of haptic shared control},
	author={Mars, Franck and Deroo, Mathieu and Hoc, Jean-Michel},
	journal={IEEE Transactions on Haptics},
	volume={7},
	number={3},
	pages={324--333},
	year={2014},
	publisher={IEEE}
}


This study investigated human-machine cooperation when driving with different degrees of a shared control system. By

means of a direct intervention on the steering wheel, shared control systems partially correct the vehicle’s trajectory and, at the same
 time, provide continuous haptic guidance to the driver. A crucial point is to determine the optimal level of steering assistance for
 effective cooperation between the two agents. Five system settings were compared with a condition in which no assistance was
 present. In addition, road visibility was manipulated by means of additional fog or self-controlled visual occlusions. Several
 performance indicators and subjective assessments were analyzed. The results show that the best repartition of control in terms of
 cooperation between human and machine can be identified through an analysis of the steering wheel reversal rate, the steering effort
 and the mean lateral position of the vehicle. The best cooperation was achieved with systems of relatively low-level haptic authority,
 although more intervention may be preferable in poor visibility conditions. Increasing haptic authority did not yield higher benefits in
 terms of steering behavior, visual demand or subjective feeling.

~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
@inproceedings{ludwig2018comparison,
	title={A comparison of concepts for control transitions from automation to human},
	author={Ludwig, Julian and Haas, Andreas and Flad, Michael and Hohmann, Soren},
	booktitle={2018 IEEE International Conference on Systems, Man, and Cybernetics (SMC)},
	pages={3201--3206},
	year={2018},
	organization={IEEE}
}

Until upcoming autonomous vehicles can handle
 every scenario in all operation domains there will be situations, in

which the human driver needs to retrieve control of the vehicle.
 This can lead to safety issues as literature shows impaired driving
 performance after taking over from highly automated driving.
 A discrete switch of control might be a valid option to hand
 over to an attentive human driver. However, it is questionable if

this is a safe way for a transition of control to somebody who is
 distracted at the time of the takeover request. Instead, gradually
 shifting control via a period of haptic shared control can provide
 guidance during the process of establishing situation awareness.
 Here, we present different design concepts for handing over
 control from a controller to a human partner. To analyze these
 concepts, we designed an experiment, in which the participants
 need to take over a simplified steering task when requested by
 the automation. We conducted a study comparing two discrete

switching transitions and three concepts in which the authority of
 the controller fades out slowly. The results show that in situations,
 needing a continuation of the control action of the automation, an
 early switch-off underperformed compared to the other concepts.
 If the situation demanded action during the transition the shared
 control approaches achieved the lowest tracking error. A survey
 of the participants revealed that gradually shifting transitions
 lead to a sense of better performance and are also regarded as
 more comfortable. The best overall results were obtained by a

concept which models human behavior and considers it within the
 takeover process. This approach provides a systematic method for
 the design of authority transitions by finding the best trade-off
 between guidance and handover.

~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

@article{marcano2020review,
	title={A review of shared control for automated vehicles: {T}heory and applications},
	author={Marcano, Mauricio and D{\'\i}az, Sergio and P{\'e}rez, Joshu{\'e} and Irigoyen, Eloy},
	journal={IEEE Transactions on Human-Machine Systems},
	volume={50},
	number={6},
	pages={475--491},
	year={2020},
	publisher={IEEE}
}

The last decade has shown an increasing interest on
 advanced driver assistance systems (ADAS) based on shared control, where automation is continuously supporting the driver at the
 control level with an adaptive authority. A first look at the literature
 offers two main research directions: 1) an ongoing effort to advance
 the theoretical comprehension of shared control, and 2) a diversity
 of automotive system applications with an increasing number of
 works in recent years. Yet, a global synthesis on these efforts is
 not available. To this end, this article covers the complete field of
 shared control in automated vehicles with an emphasis on these
 aspects: 1) concept, 2) categories, 3) algorithms, and 4) status of
 technology. Articles from the literature are classified in theory- and
 application-oriented contributions. From these, a clear distinction
 is found between coupled and uncoupled shared control. Also,
 model-based and model-free algorithms from these two categories
 are evaluated separately with a focus on systems using the steering
 wheel as the control interface. Model-based controllers tested by at
 least one real driver are tabulated to evaluate the performance of
 such systems.Results showthatthe inclusion of a driver model helps
 to reduce the conflicts at the steering. Also, variables such as driver
 state, driver effort, and safety indicators have a high impact on
 the calculation of the authority. Concerning the evaluation, driverin-the-loop simulators are the most common platforms, with few
 works performed in real vehicles. Implementation in experimental
 vehicles is expected in the upcoming years.

~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

@article{zwaan2019haptic,
	title={Haptic shared steering control with an adaptive level of authority based on time-to-line crossing},
	author={Zwaan, Hugo M and Petermeijer, Sebastiaan M and Abbink, David A},
	journal={IFAC-PapersOnLine},
	volume={52},
	number={19},
	pages={49--54},
	year={2019},
	publisher={Elsevier}
}

Traditional driver-automation interaction trades control over the vehicle back and forth between driver and automation. Haptic shared control offers an alternative by continuously sharing the control through torques on the steering wheel and pedals. When designing additional feedback torques, part of the design choice lies in the stiffness around the neutral steering point: also called the Level of Haptic Authority (LoHA), which is usually static and tuned to balance safety benefits (better at high LoHA) with conflicts torques in case of different intentions between automation and driver (higher conflict torques with increased LoHA). In this paper we explore the idea of situation-adaptive LoHA: in this case during lane-keeping by changing the LoHA based on time to lane crossing (TLC). Consequently, when safety margins are high (e.g., when driving on a wide road) the LoHA is low, but the LoHA would only increase when safety margins decrease. We propose two alternative design approaches to apply the LoHA: symmetrically and asymmetrically (i.e., only increase of LoHA in the direction of the low TLC). We compared these design in an explorative driving simulator study (n=14) to driving with two static LoHA designs (low and high). We found that compared to the high LoHA controller, both adaptive LoHA controllers designs resulted in similar safety margins, but at decreased conflict torques. Hence, a TLC-based adaptive LoHA controller seems to be an effective approach to mitigate conflicts while maintaining the safety benefits associated with HSC.

~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
@article{katzourakis2014haptic,
	title={Haptic steering support for driving near the vehicle's handling limits: Test-track case},
	author={Katzourakis, Diomidis I and Velenis, Efstathios and Holweg, Edward and Happee, Riender},
	journal={IEEE Transactions on Intelligent Transportation Systems},
	volume={15},
	number={4},
	pages={1781--1789},
	year={2014},
	publisher={IEEE}
}


Abstract—Current vehicle dynamic control systems from simple
 yaw control to high-end active steering support systems are designed to primarily actuate on the vehicle itself, rather than stimulate the driver to adapt his/her inputs for better vehicle control.
 The driver though dictates the vehicle’s motion, and centralizing
 him/her in the control loop is hypothesized to promote safety and
 driving pleasure. Exploring the above statement, the goal of this
 paper is to develop and evaluate a haptic steering support when
 driving near the vehicle’s handling limits [Haptic Support near
 the Limits (HSNL)]. The support aims to promote the driver’s
 perception of the vehicle’s behavior and handling capacity (the
 vehicle’s internal model) by providing haptic cues on the steering
 wheel. The HSNL has been evaluated in a test track where 17 test
 subjects drove around a narrow-twisting tarmac circuit, a vehicle
 (Opel Astra G/B) equipped with a steering system able to provide
 variable steering feedback torque. The drivers were instructed to
 achieve maximum velocity through corners while receiving haptic
 steering feedback cues related to the vehicle’s cornering potentials.
 The test-track tests led to the conclusion that haptic support
 reduced drivers’ mental and physical demand without affecting
 their driving performance.

==> section/preliminaries.tex <==
\section{Preliminaries}
%


==> section/prelims.tex <==
\section{Modeling the Physical Capabilities of a CAN Attacker as a Closed-Loop Attack Policy}
\label{sec:prelims}
%
In this section we briefly review a variety of security threats to automotive CAN networks that an adversary can exploit for targeting the braking ECUs (see, e.g.,~\cite{froschle2017analyzing,palanca2017stealth,miller2019lessons} for further details). This section also provides a justification for modeling the cyber-physical threat capabilities of an adversary as a closed-loop attack policy design for the vehicle actuators.

Under certain assumptions, Fr{\"o}schle and St{\"u}hring~\cite{froschle2017analyzing} have outlined a collection of six possible attacks on the CAN bus with cyber-physical implications. These attacks include: (i) blocking messages by priority; (ii) disrupting the target network; (iii) silencing a target node by dominant bits; (iv) silencing a target node by collisions; (v) suppressing a  target message; and (vi) modification attacks via either impersonating a target node or modifying target messages by suppress and inject. Through a combination of these six attacks,  Fr{\"o}schle and St{\"u}hring~\cite{froschle2017analyzing} investigate the cyber-physical implications for manipulation of steering and braking, e.g., steering a Jeep at any speed. The systemic investigation by Fr{\"o}schle and St{\"u}hring~\cite{froschle2017analyzing} was motivated by the celebrated hack of Miller and Valasek~\cite{miller2013adventures,miller2019lessons}, in which remote re-flashing of the firmware of a target microcontroller was demonstrated. 

Under the assumption of re-flashing the firmware of a target braking ECU, the adversary threat capability can be modeled by assuming complete authority over the brake actuators and full knowledge of the states of the vehicle traction dynamics by reading from the in-vehicle network, e.g., the CAN bus. \emph{In essence, the adversary can act as a feedback controller by sending malicious commands to the brake actuators while using the sensed states of the vehicle for computing these commands.}  In general, the adversary does have a very limited knowledge of the plant dynamics and its interactions with the ambient environment (vehicle traction dynamics and its interaction with the road). Consequently, the closed-loop attack policies on a vehicle actuator can be located within the cyber-physical attack space due to Teixeira \emph{et al.}~\cite{teixeira2015secure} according to Figure~\ref{fig:newFig}(right).  %provides a  classification of the proposed attack policy in this paper by  
 %
%In this section we provide some preliminary definitions from finite-time stability theory. The interested reader is referred to~\cite{polyakov2014stability,zhou2016asymptotic,sanchez2015predefined,polyakov2015finite,song2019time} for further details. 
%
%Consider the dynamical system
%%
%\begin{equation}
%\dot{y} = f(t,y;\zeta)
%\label{eq:prelim1}
%\end{equation}
%% 
%where $t\in [t_0, \infty)$ for some $t_0>0$, $y\in \mathbb{R}^n$, and $\zeta \in \mathbb{R}^m$ denote time, the state, and the parameters of the system in~\eqref{eq:prelim1}, respectively. We denote the solutions to~\eqref{eq:prelim1} starting from $y_0=y(t_0)$  by $y(t,y_0)$. We say that the non-empty set $\Gamma \subset \mathbb{R}^n$ is \emph{locally finite-time stable}  for~\eqref{eq:prelim1} if $\Gamma$ is locally asymptotically stable for~\eqref{eq:prelim1} and there exists a neighborhood of $\Gamma$, denoted by $\mathcal{N}(\Gamma)$, such that any solution $y(t,y_0)$ of~\eqref{eq:prelim1} with $y_0\in \mathcal{N}(\Gamma)$  reaches $\Gamma$ in a finite time moment $t^\ast=T(y_0)$, where the \emph{settling-time function} $T: \mathcal{N}(\Gamma) \to \rpos$ is locally bounded. We say that~\eqref{eq:prelim1} is \emph{locally fixed-time stable} if it is locally finite-time stable and there exists some positive constant $T_{max}$, called the \emph{settling-time}, such that $T(y_0) \leq T_{max}$ for all $y_0\in \mathcal{N}(\Gamma)$. If $\mathcal{N}(\Gamma) = \mathbb{R}^n$, the definitions will become global. 

%We denote the set of non-negative real numbers by $\mathbb{R}_{\geq 0}$. Following the notation in~\cite{zhou2016asymptotic}, given the interval $J=[t_0,\infty)\subset \mathbb{R}_{\geq 0}$ where $t_0$ is some positive real number, we let $\mathbb{PC}(J,\mathbb{R})$ denote the union of the sets of all real-valued piecewise continuous and continuously differentiable functions defined on $J$. Consider the LTV system 
%%
%\begin{equation}
%\dot{x} = a(t) x(t), 
%\label{eq:prelim2}
%\end{equation}
%% 
%where $a(.) \in \mathbb{PC}(J,\mathbb{R})$ and $x\in \mathbb{R}$. We say that the LTV system in~\eqref{eq:prelim2} is \emph{uniformly exponentially stable} if there exist positive constants $\gamma$ and $k$ such that $|x(t)| \leq k |x(t_0)| \exp(-\gamma (t-t_0) )$ for all $t, t_0 \in J$ with $t\geq t_0$.
 

==> section/zerodyn.tex <==



